Autonomous Aerial Cinematography In Unstructured Environments With Learned Artistic Decision-Making

Aerial cinematography is revolutionizing industries that require live and dynamic camera viewpoints such as entertainment, sports, and security. However, safely piloting a drone while filming a moving target in the presence of obstacles is immensely taxing, often requiring multiple expert human operators. Hence, there is demand for an autonomous cinematographer that can reason about both geometry and scene context in real-time. Existing approaches do not address all aspects of this problem; they either require high-precision motion-capture systems or GPS tags to localize targets, rely on prior maps of the environment, plan for short time horizons, or only follow artistic guidelines specified before flight. In this work, we address the problem in its entirety and propose a complete system for real-time aerial cinematography that for the first time combines: (1) vision-based target estimation; (2) 3D signed-distance mapping for occlusion estimation; (3) efficient trajectory optimization for long time-horizon camera motion; and (4) learning-based artistic shot selection. We extensively evaluate our system both in simulation and in field experiments by filming dynamic targets moving through unstructured environments. Our results indicate that our system can operate reliably in the real world without restrictive assumptions. We also provide in-depth analysis and discussions for each module, with the hope that our design tradeoffs can generalize to other related applications. Videos of the complete system can be found at: https://youtu.be/ookhHnqmlaU.

==> inputs/99_approach.tex <==
% !TEX root = ../root.tex

\section{Approach} 
\label{sec:approach}

\rbnote{get rid of approach and just make one section for each main area}

\rbnote{add section on shot selection}

We now detail our approach for each sub-system of the aerial cinematography platform. At a high-level, three main sub-systems operate together: (A) Vision, required for localizing the target's position and orientation and for recording the final UAV's footage; (B) Mapping, required for creating an environment representation; and (C) Planning, which combines the actor's pose and the environment to calculate the UAV trajectory. Fig.~\ref{fig:system2} shows a system diagram.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/diagram_new}
    \caption{System architecture. Vision subsystem controls camera's orientation and forecasts the actor trajectory $\Path{a}$ using  monocular images. Mapping receives LiDAR pointclouds to incrementally calculate a truncated signed distance transform (TSDT). Planning uses the map, the drone's state estimation and actor's forecast to generate trajectories for the flight controller.}
    \label{fig:system2}
\end{figure}

\input{inputs/4_vision}
\input{inputs/4_mapping}
\input{inputs/4_planning}

==> inputs/99_setup.tex <==
% !TEX root = ../root.tex

\subsection{Experimental setup}
\label{subsec:experiments_setup}





% \missingfigure[figwidth=0.5\textwidth]{New system setup w/ velodyne}
% \rbnote{talk about testing location?}

% Our drone is the DJI M210 model, coupled with a NVIDIA TX2 computer for both vision and planning pipelines (Figure~\ref{fig:system2}). \chnote{comment on camera}
% \chnote{go into more details on the TX2, how many cores, what processor and RAM}
% ROS~\citep{ros2018} infrastructure handles node communication. 
% In the vision pipeline, we detect the actor using Faster-RCNN~\citep{ren2015faster} with MobileNets \citep{howard2017mobilenets} for feature extraction and Kernelized Correlation Filter (KCF)~\citep{henriques2015high} for tracking, controlling the camera gimbal to keep the actor within the desired screen position. 
% The actor wears a Pixhawk PX4 module on a hat that sends his pose to the onboard computer via radio communication.
% , and in other experiments we use a purely visual actor localization and heading estimation. 

% A linear Kalman filter uses these pose estimates to infer his velocity, which is used to predict her trajectory ($\Path{a}$) for the next 10 s. Using a point cloud map of the test site we pre-compute a TSDF map of the region of interest. 
% Re-planning happens at 5 Hz with a 10 s horizon. 

% To simulate the full pipeline and to decide on the relative weights between each cost function (Eq.~\ref{eq:rel_cost}), we built a ROS wrapper to test our software in a photo-realistic environment \cite{airsim2017fsr} (Fig.~\ref{fig:simulator}).

% \begin{figure}[b]
%     \includegraphics[width=0.55\textwidth]{figs/sim.png}
%     \caption{Photo-realistic simulator used to test the system. Third and first-person renderings shown on the left, and occupancy map with drone trajectory shown on the right.}
%     \label{fig:simulator}
% \end{figure}




==> inputs/99_stats.tex <==
% !TEX root = ../root.tex

\subsection{System statistics}
\label{subsec:experiments_stats}

% \rbnote{show useful statistics about system performance that allows us to get useful insights into bottlenecks and give others an idea of what needs improvement in the future}

\chnote{incorporate time takes for one laser scan update, maybe a time statistic table?}
% \rbnote{include stats on: flight time, planning freq, plan time horizon, num iterations max, how much \% of CPU, GPU and RAM each sub-system is taking, time that it takes to update one laser scan}
% \begin{table}[]
%     \caption{Planning parameters used in experiments \chnote{RB: pls confirm values}}
%     \begin{tabular}{l|l}
%     \hline
%     \textbf{Parameter} & \textbf{Value} \\ \hline
%     Planning Freq. & 5 Hz \\
%     Max. Iteration & 100? \\
%     Planning time horizon & 5s \\ \hline
%     \end{tabular}
%     \label{table:planning_param}
% \end{table}
\begin{table}[ht]
        \caption{Planning parameters used in experiments \chnote{step size}}

    \begin{tabular}{llll}
    \hline
    \textbf{Parameter} & Planning Freq. & Max. Iteration & Planning time horizon \\ \hline
    \textbf{Value} & \multicolumn{1}{c}{5Hz} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{10s} \\ \hline
    \end{tabular}
    \label{tab:planning_param}
\end{table}

\begin{table}[ht]
    \caption{Compute Statistics \chnote{add footnotes about detect/track, heading only when tracking}}
    \begin{tabular}{cc|ccc}
        \hline
        \textbf{Subsystem} & \textbf{Module} & \textbf{\% Thread} & \textbf{\% GPU} & \textbf{\% RAM} \\ \hline
        Vision & \begin{tabular}[c]{@{}c@{}}Detection/Tracking\\ Gimbal Control\\ Heading Est.\\ KF\end{tabular} & \begin{tabular}[c]{@{}c@{}}56.6/24.2\\ 9.9\\ 23.5\\ 8.2\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}27.0/0.3\\ 0.6\\ 22.3\\ 1.0\end{tabular} \\ \hline
        Mapping & \begin{tabular}[c]{@{}c@{}}Dist. TF Map\\ Occupancy Map\\ LiDAR Driver\end{tabular} & \begin{tabular}[c]{@{}c@{}}91.0\\ 22.3\\ 23.5\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}9.5\\ 0.6\\ 0.1\end{tabular} \\ \hline
        Planning & CHOMP & 98.3 &  & 9.5 \\ \hline
        Hardware & DJI SDK & 89.7 &  & 0.5
        \end{tabular}
    
\end{table}

\rbnote{add runtime for each module as well? how long it takes (ms) for each part to complete a cycle}

\missingfigure[figwidth=0.5\textwidth]{Time needed for Distance Transform Update over Flight Time. Time decreases as less cells will be updated.}

% \rbnote{maybe say a few tricks I had to do when switching from offline to online map? such as had to significantly decrease threshold for signed distance calculation from 10m to 4m to make computation feasible, and had to significantly lower num of iterations for planner and increase step size to get to solutions much faster and keep re-planning at 5Hz}
